Continuous Learning from Executable Environments: Autonomous Skill Acquisition, Retention, and Transfer in Language Models

A language model does not keep the experience of a task it completes. Where an attempt can be checked by executing it, that experience can become training data without human-written tasks or labels. We present and evaluate a framework that generates practice tasks, verifies attempts by execution, trains a small adapter (added weights; the base model remains fixed) on the verified records, and repeats, one generation per repetition, evaluating every model on a held-out examination that no stage of the pipeline reads. In predicting the output of Lua programs, using an interpreter as the sole source of labels, a 4-billion-parameter (4B) model's examination accuracy rises from 5.05% to 13.24% over four generations. In editing files with Vim, a larger teacher model writes tasks from the user manual and supplies most verified solutions. Trained on these records, the 4B model solves hand-written examination tasks its base never solves (up to 3.50% of attempts, versus 62.25% for the teacher), whereas a control trained with mismatched task requests solves none. On 228 easier hand-written course exercises, the pass rate rises from 15-16% to 37-41% (exploratory). An iterative protocol then ran three generations with 4B and 8B models, governing every release by a fixed rule. In the first generation, examination gains were one-tenth to one-fifth of the gains on held-out generated tasks. Across training seeds, later candidates averaged 1.2 to 6.1 percentage points above their baselines on generated tasks, implying an expected examination gain of 0.1 to 1.3 points, below the 100-task examination's 2.8-point detection threshold. Consequently, no later examination gain was established, and because outcomes were recorded per attempt rather than per task, whether transfer, acquisition, or retention stalled remains undecided.

==> generated/artifacts.tex <==
dataset & \href{https://huggingface.co/datasets/swedishembedded/vim-headless-mastery}{\nolinkurl{swedishembedded/vim-headless-mastery}} & \texttt{ff83d49b1b7d} & public & the hand-written Vim course: its single-idea exercises and the examination tasks, with their checks and reference answers (the composite course exercises are not published) \\
dataset & \href{https://huggingface.co/datasets/swedishembedded/vim-headless-mastery-manual}{\nolinkurl{swedishembedded/vim-headless-mastery-manual}} & \texttt{e3ee7a458c06} & private & the tasks authored from the user manual in both authoring modes and for the later generations, held-out tasks included \\
dataset & \href{https://huggingface.co/datasets/swedishembedded/vim-headless-mastery-sft-manual}{\nolinkurl{swedishembedded/vim-headless-mastery-sft-manual}} & \texttt{bc55f91f923f} & private & verified trajectories of teacher and learner on the authored tasks, with every graded attempt and its reward \\
dataset & \href{https://huggingface.co/datasets/swedishembedded/vim-headless-mastery-sft}{\nolinkurl{swedishembedded/vim-headless-mastery-sft}} & \texttt{303ba2e401c2} & public & the training trajectories of the all-verified and outcome-first conditions as chat records, without the records of the held-out tasks; and, as its default configuration, teacher trajectories on the course's exercises, on which no model of this paper was trained \\
dataset & \href{https://huggingface.co/datasets/swedishembedded/vim-headless-mastery-sft-g2}{\nolinkurl{swedishembedded/vim-headless-mastery-sft-g2}} & \texttt{f0b91d2b7700} & private & a second generation of the course-exercise trajectories, not used by any model of this paper \\
model & \href{https://huggingface.co/swedishembedded/vim-manual-transfer-adapters}{\nolinkurl{swedishembedded/vim-manual-transfer-adapters}} & \texttt{0485d8a1e2a8} & private & the adapters of the training-material experiment (six conditions, three seeds) and one seed of the first 8B generation of the earlier iterative runs; the adapters of the iterative protocol and of its replications were not retained \\
model & \href{https://huggingface.co/swedishembedded/vim-headless-mastery-sft-adapters}{\nolinkurl{swedishembedded/vim-headless-mastery-sft-adapters}} & \texttt{6f095d355423} & private & adapters trained on the course-exercise trajectories, not evaluated in this paper \\
model & \href{https://huggingface.co/Qwen/Qwen3-4B}{\nolinkurl{Qwen/Qwen3-4B}} & \texttt{1cfa9a720891} & public & the 4B learner and base \\
model & \href{https://huggingface.co/Qwen/Qwen3-8B}{\nolinkurl{Qwen/Qwen3-8B}} & \texttt{ada7b65d0f3b} & public & the 8B learner; the revision is the checkpoint digest (the download revision was not recorded) \\
model & \href{https://huggingface.co/Qwen/Qwen3.8-27B-FP8}{\nolinkurl{Qwen/Qwen3.8-27B-FP8}} & \texttt{c3a462cc3d38} & public & the Vim task author and teacher \\
evidence & \href{https://huggingface.co/datasets/swedishembedded/source-to-transfer-evidence}{\nolinkurl{swedishembedded/source-to-transfer-evidence}} & \texttt{af066f369fb2} & private & Vim aggregates and decisions, the evaluation records of the iterative protocol and its training-step replications, training sets with lineage, run manifests, analysis code and figure data \\
evidence & \href{https://huggingface.co/datasets/swedishembedded/generalized-continuous-learning-evidence}{\nolinkurl{swedishembedded/generalized-continuous-learning-evidence}} & \texttt{34a2c5bbc62d} & private & Lua adapters, lineage records and the examiner's verdicts \\
code & \href{https://github.com/swedishembedded/splinter}{\nolinkurl{swedishembedded/splinter}} & \texttt{578cfec9b} & public & the learning controller \\
code & \href{https://github.com/swedishembedded/sven}{\nolinkurl{swedishembedded/sven}} & \texttt{704496d62} & public & the agent that makes each attempt \\
code & \href{https://github.com/swedishembedded/brain}{\nolinkurl{swedishembedded/brain}} & \texttt{b2f46a22c} & public & model serving and adapter training \\
materials & \href{\MaterialsRepo}{\nolinkurl{\MaterialsName}} & \texttt{\MaterialsCommitShort} & public & the Vim task environment, the authoring prompts, schemas and operators, the recipes (both authoring modes, the training-material conditions, the course-exercise evaluations, the three generations of the iterative protocol), the evaluation plans, the Lua prediction environment with its examination generator and check, and the examiner; GPL-3.0-only \\


==> generated/builds.tex <==
splinter & \texttt{f6661e34be6b} & \texttt{splinter-f6661e34b/splinter} & \texttt{aa162ad978cfab42} & Vim training-material experiment: datasets, training, evaluations \\
splinter & \texttt{cc5581333a14} & \texttt{splinter-cc5581333/splinter} & \texttt{eb814939016bbf04} & Vim authoring run, attempt stages \\
splinter & \texttt{d3ab644fafa2} & \texttt{splinter-d3ab644fa/splinter} & \texttt{faa5b47e3b360d9a} & Vim authoring run, authoring stages \\
brain & \texttt{b726c045bb34}\newline (\texttt{d6bd3baaff53}) & \texttt{brain-b726c045b/brain} & \texttt{0d62d4c7ae404664} & Vim serving and training of the training-material experiment \\
brain & \texttt{b726c045bb34}\newline (\texttt{d6bd3baaff53}) & \texttt{brain-b726c045b/brain-gpu-worker} & \texttt{ab5c2e8692370fed} & as above \\
brain & \texttt{2104ee58f960} & \texttt{brain-2104ee58f/brain} & \texttt{02d475dd9fdb6a44} & Vim serving of the iterative runs on part of the nodes: the router spreads an adapter's requests \\
brain & \texttt{2104ee58f960} & \texttt{brain-2104ee58f/brain-gpu-worker} & \texttt{62947d0d5d8600c1} & as above \\
brain & \texttt{62821de326bd} & \texttt{brain-62821de32/brain} & \texttt{0b694249e8fb6ae4} & Vim authoring run, attempt stages \\
brain & \texttt{62821de326bd} & \texttt{brain-62821de32/brain-gpu-worker} & \texttt{ab5c2e8692370fed} & as above \\
sven & \texttt{01eabb507058} & \texttt{sven-01eabb507/sven} & \texttt{d63fc391f8ac687c} & the agent of every Vim attempt \\
sven & \texttt{704496d626cb} & \texttt{(library)} & \texttt{} & the agent library linked into the learning controller in every run \\
splinter & \texttt{578cfec9b931} & \texttt{(source revision)} & \texttt{} & the iterative protocol and its training-step replications \\
brain & \texttt{b2f46a22c879} & \texttt{(source revision)} & \texttt{} & serving and training of the iterative protocol \\
splinter & \texttt{2fd05cc42a70} & \texttt{(source revision)} & \texttt{} & used once, by hand, to remove the sandbox of one finished attempt \\


==> generated/claims-table.tex <==
\texttt{lua-early-steps} & Do the first two Lua generations each improve on their predecessor on the independent examination? & program family and lineage (examiner's bootstrap) & primary & improvement supported \\
\texttt{lua-late-steps} & Do Lua generations 3 and 4 each improve on their predecessor? & program family and lineage (examiner's bootstrap) & primary & inconclusive \\
\texttt{lua-total-gain} & Does Lua generation 4 improve on the base on the independent examination? & program family and lineage (examiner's bootstrap) & primary & improvement supported \\
\texttt{lua-new-families} & Does the Lua gain extend to program families never used in any examination before? & program family and lineage (examiner's bootstrap) & primary & improvement supported \\
\texttt{vim-transfer-arms} & Do trajectories on automatically authored Vim tasks teach a 4B model skills it applies to the independent examination? & task (examination task), passes pooled over three training seeds & primary & improvement supported \\
\texttt{vim-heldout-arms} & Do the training-material conditions improve on held-out generated tasks? & task (held-out generated task), passes pooled over three seeds & secondary & improvement supported \\
\texttt{vim-practice-transfer-4b} & Do first-generation 4B candidates pass more of the hand-written course exercises, which nothing was trained on, than their base? & task (course exercise) & no & improvement supported \\
\texttt{vim-practice-transfer-8b} & Do first-generation 8B candidates pass more of the hand-written course exercises, which nothing was trained on, than their base? & task (course exercise) & no & improvement supported \\
\texttt{vim-outcome-first} & Does outcome-first authoring transfer more than section-by-section authoring? & task (examination task), passes pooled over three seeds & secondary & improvement supported \\
\texttt{vim-shuffled-control} & Does the shuffled-request control pass examination attempts its base does not? (It is the reference of vim-transfer-arms; a control that passes nothing cannot be supported as an improvement.) & task (examination task) & no & inconclusive \\
\texttt{vim-learner-only} & Does training on the learner's own verified successes alone transfer to the examination? & task (examination task), passes pooled over three seeds & no & excluded \\
\texttt{vim-a-exam-4b-g1} & Earlier iterative runs: does 4B generation 1 beat the base on the examination? & task (examination task) & primary & improvement supported \\
\texttt{vim-a-exam-8b-g1} & Earlier iterative runs: does 8B generation 1 beat the base on the examination? & task (examination task) & primary & excluded \\
\texttt{vim-a-exam-g2} & Earlier iterative runs: does generation 2 beat generation 1 on the examination? & task (examination task) & primary & inconclusive \\
\texttt{vim-b-heldout-g1} & Iterative protocol: does generation 1 beat the base on held-out generated tasks? & attempt slot as recorded; the registered unit is the task, bounded from the slot counts & no & improvement supported \\
\texttt{vim-b-heldout-steps-8b} & Iterative protocol, 8B: do generations 2 and 3 each beat their champion on held-out generated tasks? & attempt slot as recorded; the registered unit is the task, bounded from the slot counts & no & inconclusive \\
\texttt{vim-b-heldout-steps-4b} & Iterative protocol, 4B: do generations 2 and 3 each beat their champion on held-out generated tasks? & attempt slot as recorded; the registered unit is the task, bounded from the slot counts & no & inconclusive \\
\texttt{vim-b-exam-8b-g1} & Iterative protocol: does 8B generation 1 beat the base on the examination? & attempt slot as recorded; the registered unit is the task, bounded from the slot counts & secondary & excluded \\
\texttt{vim-b-exam-4b-g1} & Iterative protocol: does 4B generation 1 beat the base on the examination? & attempt slot as recorded; the registered unit is the task, bounded from the slot counts & secondary & inconclusive \\
\texttt{vim-b-exam-steps} & Iterative protocol: does a later generation beat its champion on the examination? & attempt slot as recorded; the registered unit is the task, bounded from the slot counts & primary & inconclusive \\
\texttt{vim-br-heldout} & Training-step replications: do the steps improve on held-out generated tasks over seeds? & attempt slot summed over training seeds that share tasks and one champion measurement: not independent units, no valid test & secondary & inconclusive \\
\texttt{vim-br-exam} & Training-step replications: do the steps improve on the examination over seeds? & attempt slot summed over training seeds that share tasks and one champion measurement: not independent units, no valid test & secondary & inconclusive \\
\texttt{vim-a-retention} & Earlier iterative runs: does generation 2 retain generation 1's held-out tasks? & task (held-out generated task) & no & retention supported \\
\texttt{vim-b-retention} & Iterative protocol: do the candidates retain earlier generations' held-out tasks? & attempt slot as recorded; the registered unit is the task, bounded from the slot counts & no & inconclusive \\
\texttt{vim-practice-retention-4b} & Do the 4B generation-1 candidates retain the base's competence on hand-written course exercises? & task (course exercise) & no & retention supported \\
\texttt{vim-practice-retention-8b} & Do the 8B first-generation candidates retain the base's competence on hand-written course exercises, in every evaluation within the bound on uncounted attempts? & task (course exercise) & no & retention supported \\
\texttt{learning-efficiency} & Does learning make further learning cheaper? & generation & no & inconclusive \\
\texttt{eng-generate-tasks} & Was executable practice material generated without hand-written tasks? & count in the evidence & no & exercised \\
\texttt{eng-reject-invalid} & Were invalid generated tasks rejected automatically? & count in the evidence & no & exercised \\
\texttt{eng-verified-solutions} & Were verified solutions produced for the admitted tasks? & count in the evidence & no & exercised \\
\texttt{eng-training-material} & Were verified solutions converted to training records? & count in the evidence & no & exercised \\
\texttt{eng-train-adapters} & Were adapters trained locally on those records? & count in the evidence & no & exercised \\
\texttt{eng-independent-evaluation} & Were candidates evaluated on tasks outside the training and release loop? & count in the evidence & no & exercised \\
\texttt{eng-successive-generations} & Did successive generations run and release in the iterative protocol with no person deciding between them? & count in the evidence & no & exercised \\
\texttt{eng-accept-reject} & Did the release rule both accept and reject candidates? & count in the evidence & no & exercised \\
\texttt{eng-measure-earlier} & Were earlier generations' tasks re-measured for every later candidate? & count in the evidence & no & exercised \\


==> generated/compute-accounting.tex <==
Lua generation 1 & 4 lineages, one card each & 5100 programs proposed, 4000 records trained, 1000 steps & 2.99 \\
Lua generation 2 & 4 lineages, one card each & 9300 programs proposed, 8000 records trained, 2000 steps & 2.25 \\
Lua generation 3 & 4 lineages, one card each & 18600 programs proposed, 16000 records trained, 4000 steps & 4.31 \\
Lua generation 4 & 4 lineages, one card each & 39506 programs proposed, 32000 records trained, 8000 steps & 11.90 \\
Vim training, condition all verified & 3 seeds, one card each & 3739 training and validation records, 2400 steps completed, 82.6M row tokens & 2.56 \\
Vim training, condition one per task & 3 seeds, one card each & 857 training and validation records, 1760 steps completed, 47.1M row tokens & 0.86 \\
Vim training, condition productive actions & 3 seeds, one card each & 3739 training and validation records, 2400 steps completed, 82.3M row tokens & 2.53 \\
Vim training, condition shuffled requests & 3 seeds, one card each & 3739 training and validation records, 2400 steps completed, 83.4M row tokens & 2.55 \\
Vim training, condition outcome first & 3 seeds, one card each & 1230 training and validation records, 2280 steps completed, 80.2M row tokens & 2.05 \\
Vim authoring (outcome first): admission replay & several cards behind a router & 467 attempts, 467 physical attempts, 467 counted, 467 verified & not recorded \\
Vim authoring (outcome first): teacher reaching the end states & several cards behind a router & 2820 attempts, 3799 physical attempts, 2805 counted, 1387 verified & not recorded \\
Vim authoring (outcome first): learner attempts & several cards behind a router & 3736 attempts, 4091 physical attempts, 3688 counted, 116 verified & not recorded \\
Vim authoring (outcome first): teacher attempts & several cards behind a router & 1868 attempts, 1875 physical attempts, 1868 counted, 1348 verified & not recorded \\
Vim authoring (section by section): admission replay & several cards behind a router & 1030 attempts, 1030 physical attempts, 1030 counted, 1026 verified & not recorded \\
Vim authoring (section by section): learner attempts & several cards behind a router & 8208 attempts, 8533 physical attempts, 8204 counted, 824 verified & not recorded \\
Vim authoring (section by section): teacher attempts & several cards behind a router & 4104 attempts, 4113 physical attempts, 4095 counted, 3319 verified & not recorded \\
Vim evaluation, earlier iterative runs & several cards behind a router & 7896 attempts scheduled & not recorded \\
Vim evaluation, iterative protocol & several cards behind a router & 9776 attempts scheduled & not recorded \\
Vim evaluation, training-step replications (new candidates only) & several cards behind a router & 11732 attempts scheduled & not recorded \\


==> generated/compute-missing.tex <==
evaluation accelerator time & every Vim evaluation stage (the training-material experiment, the iterative protocol and its replications, the earlier runs, the course exercises) and the Lua examiner & evaluation results hold counts of attempts, not durations or the cards that served them \\
rollout accelerator time & learner, teacher, admission-replay and outcome-reproduction attempt stages of both authoring runs & the attempt reports hold attempts, physical attempts and statuses, not durations; requests were routed over several cards \\
rollout tokens & every agent rollout (authoring attempts and evaluations) & prompt and completion tokens per attempt are not in the attempt reports or evaluation results \\
rollout tool calls & every agent rollout & tool-call counts per attempt are in the private attempt data only \\
authoring tokens & task proposal, review and repair by the task author, both authoring modes & the stage manifests hold item counts and rejections, not token usage or durations \\
sandbox time & admission by replay and replay verification & executions are counted; their durations are not recorded in the published reports \\
earlier-run training time & generation 2 and the 8B generation-1 adapters of the earlier iterative runs & their training reports are not in the evidence dataset (only the fifteen runs of the training-material experiment are); the 4B generation 1 is the outcome-first condition's seed 3 and is covered \\
iterative-protocol training time & generations 1 to 3 at both sizes and every training-step replication & the records hold evaluation counts and revisions only; the run directories no longer exist \\
iterative-protocol steps, epochs and records per generation & the iterative protocol and its training-step replications & stated in the registration (budget 1.9 epochs) but no training report is in the evidence, so steps completed and records are not verifiable from it \\
generation wall clock with the accelerators engaged & the iterative protocol and the earlier iterative runs & elapsed times are in no evidence file, and the number of cards engaged per stage is not recorded: elapsed time on several cards is not accelerator-hours \\
infrastructure overhead & queueing, retries and failures of every run & only uncounted slots and physical attempts per stage are recorded; no queue or retry timing \\
learning efficiency & improvement per accelerator-hour or per token, per generation & needs the missing evaluation, rollout and iterative-protocol training costs; computable only for the Lua generations and the trainings of the training-material experiment, which have no matched cost of their transfer \\


==> generated/iterative-steps.tex <==
8B generation 1 vs base & own held-out tasks & 85/224 & 9/224 & $+33.93$ & 79/3 & \ensuremath{1.4\times 10^{-17}} to 0.00024 & improvement supported \\
8B generation 1 vs base & examination & 25/400 & 0/391 & $+6.25$ & 25/0 & \ensuremath{3.0\times 10^{-8}} to 0.0078 & excluded \\
8B generation 2 vs generation 1 & own held-out tasks & 55/188 & 40/188 & $+7.98$ & 29/14 & \ensuremath{4.2\times 10^{-6}} to 0.942 & inconclusive \\
8B generation 2 vs generation 1 & generation 1 held-out tasks & 92/224 & 86/224 & $+2.68$ & 29/23 & \ensuremath{5.8\times 10^{-5}} to 0.999 & inconclusive \\
8B generation 2 vs generation 1 & examination & 30/400 & 30/400 & $+0.00$ & 17/17 & 0.0059 to 1 & inconclusive \\
8B generation 3 vs generation 2 & own held-out tasks & 59/196 & 45/196 & $+7.14$ & 25/11 & \ensuremath{1.4\times 10^{-5}} to 0.895 & inconclusive \\
8B generation 3 vs generation 2 & generation 2 held-out tasks & 49/188 & 54/188 & $-2.66$ & 14/19 & 0.032 to 1 & inconclusive \\
8B generation 3 vs generation 2 & generation 1 held-out tasks & 109/224 & 105/224 & $+1.79$ & 18/14 & 0.0022 to 0.99 & inconclusive \\
8B generation 3 vs generation 2 & examination & 32/400 & 32/400 & $+0.00$ & 18/18 & 0.0053 to 1 & inconclusive \\
4B generation 1 vs base & own held-out tasks & 64/224 & 6/222 & $+25.87$ & 62/4 & \ensuremath{1.4\times 10^{-17}} to 0.0059 & improvement supported \\
4B generation 1 vs base & examination & 11/400 & 0/397 & $+2.75$ & 11/0 & 0.00049 to 0.125 & inconclusive \\
4B generation 2 vs generation 1 & own held-out tasks & 35/188 & 31/188 & $+2.13$ & 17/13 & 0.0022 to 0.989 & inconclusive \\
4B generation 2 vs generation 1 & generation 1 held-out tasks & 76/224 & 68/224 & $+3.57$ & 27/19 & \ensuremath{5.7\times 10^{-5}} to 0.995 & inconclusive \\
4B generation 2 vs generation 1 & examination & 11/400 & 12/400 & $-0.25$ & 10/11 & 0.046 to 1 & inconclusive \\
4B generation 3 vs generation 1 & own held-out tasks & 41/196 & 27/196 & $+7.14$ & 24/10 & \ensuremath{1.8\times 10^{-5}} to 0.895 & inconclusive \\
4B generation 3 vs generation 1 & generation 2 held-out tasks & 30/188 & 31/188 & $-0.53$ & 11/12 & 0.029 to 1 & inconclusive \\
4B generation 3 vs generation 1 & generation 1 held-out tasks & 83/224 & 68/224 & $+6.70$ & 28/13 & \ensuremath{4.2\times 10^{-6}} to 0.942 & inconclusive \\
4B generation 3 vs generation 1 & examination & 13/400 & 12/400 & $+0.25$ & 11/10 & 0.029 to 0.989 & inconclusive \\


==> generated/ledger.tex <==
Generate practice tasks, reject invalid ones, verify solutions by execution, build training sets, train adapters, evaluate outside the pipeline, run successive generations with releases decided by rule, re-measure earlier tasks & exercised \\
Improve interpreter-based examination accuracy & supported \\
Extend that gain to program families never examined before & supported \\
Acquire transferable Vim capabilities & supported, under the tested conditions \\
Transfer to hand-written course exercises & supported (exploratory) \\
Retain earlier capabilities across generations & release rule satisfied; not established \\
Continue improving on held-out generated tasks & observed higher; not established \\
Continue improving on the independent examination & not established \\
Improve efficiency of acquiring new skills & not established \\


==> generated/lua-steps.tex <==
Generation 1 vs base & 10.12\% & 5.05\% & $+5.07$ [$+2.60$, $+7.76$] & improvement supported \\
Generation 2 vs 1 & 11.72\% & 10.12\% & $+1.59$ [$+0.12$, $+3.33$] & improvement supported \\
Generation 3 vs 2 & 12.95\% & 11.72\% & $+1.24$ [$-0.36$, $+2.98$] & inconclusive \\
Generation 4 vs 3 & 13.24\% & 12.95\% & $+0.28$ [$-1.54$, $+2.24$] & inconclusive \\
Generation 4 vs base & 13.24\% & 5.05\% & $+8.19$ [$+5.12$, $+11.52$] & improvement supported \\
\quad never-examined families & 4.63\% & 1.38\% & $+3.25$ [$+0.66$, $+7.10$] & improvement supported \\
\quad families examined before & 19.64\% & 7.78\% & $+11.86$ [$+7.01$, $+17.09$] & improvement supported \\


==> generated/replication-steps.tex <==
8B generation 2 & own held-out tasks & 4 & 55, 51, 51, 49 & 40/188 & 4/0 & 99/53 & inconclusive \\
8B generation 2 & generation 1 held-out tasks & 4 & 92, 91, 96, 96 & 86/224 & 4/0 & 115/84 & inconclusive \\
8B generation 2 & examination & 4 & 30, 27, 29, 33 & 30/400 & 1/2 & 63/64 & inconclusive \\
8B generation 3 & own held-out tasks & 3 & 59, 51, 54 & 45/196 & 3/0 & 64/35 & inconclusive \\
8B generation 3 & generation 2 held-out tasks & 3 & 49, 57, 58 & 54/188 & 2/1 & 61/59 & inconclusive \\
8B generation 3 & generation 1 held-out tasks & 3 & 109, 106, 104 & 105/224 & 2/1 & 52/48 & inconclusive \\
8B generation 3 & examination & 3 & 32, 37, 36 & 32/400 & 2/0 & 66/57 & inconclusive \\
4B generation 2 & own held-out tasks & 5 & 35, 33, 32, 41, 25 & 31/188 & 4/1 & 76/65 & inconclusive \\
4B generation 2 & generation 1 held-out tasks & 5 & 76, 83, 88, 85, 78 & 68/224 & 5/0 & 154/84 & inconclusive \\
4B generation 2 & examination & 5 & 11, 13, 18, 17, 13 & 12/400 & 4/1 & 58/46 & inconclusive \\
4B generation 3 & own held-out tasks & 5 & 41, 34, 33, 37, 41 & 27/196 & 5/0 & 102/51 & inconclusive \\
4B generation 3 & generation 2 held-out tasks & 5 & 30, 41, 38, 38, 40 & 31/188 & 4/1 & 88/56 & inconclusive \\
4B generation 3 & generation 1 held-out tasks & 5 & 83, 75, 96, 89, 95 & 68/224 & 5/0 & 172/74 & inconclusive \\
4B generation 3 & examination & 5 & 13, 16, 14, 17, 12 & 12/400 & 4/0 & 56/44 & inconclusive \\


==> generated/retention.tex <==
4B outcome first, seed 3 & 378/912 & 138/912 & 120/16, \ensuremath{3.5\times 10^{-21}} & $+26.32$ [$+21.38$, $+31.47$] \\
4B productive actions, seed 1 & 360/912 & 141/910 & 109/13, \ensuremath{2.3\times 10^{-20}} & $+24.07$ [$+19.10$, $+28.98$] \\
4B one per task, seed 1 & 336/912 & 142/912 & 103/17, \ensuremath{1.7\times 10^{-16}} & $+21.27$ [$+16.45$, $+26.32$] \\
8B generation 1, seed 1\textsuperscript{a} & 463/912 & 139/893 & 129/14, \ensuremath{8.9\times 10^{-25}} & $+36.06$ [$+30.49$, $+41.53$] \\
8B generation 1, seed 2 & 461/908 & 138/903 & 138/10, \ensuremath{3.1\times 10^{-30}} & $+35.77$ [$+30.45$, $+40.99$] \\
8B generation 1, seed 3 & 408/912 & 134/897 & 127/14, \ensuremath{2.9\times 10^{-24}} & $+30.32$ [$+25.42$, $+35.35$] \\


==> generated/transfer-projection.tex <==
8B generation 2 & $+6.12$ & $+0.65$ to $+1.25$ & $-0.06$ & $-0.75$ to $+0.75$ & $-3.7$ to $+3.7$ & $3.6$ & 840 to 3\,100 \\
8B generation 3 & $+4.93$ & $+0.52$ to $+1.01$ & $+0.75$ & $+0.00$ to $+1.25$ & $-3.8$ to $+3.8$ & $3.7$ & 1\,400 to 5\,100 \\
4B generation 2 & $+1.17$ & $+0.12$ to $+0.24$ & $+0.60$ & $-0.25$ to $+1.50$ & $-2.7$ to $+2.2$ & $2.8$ & 14\,000 to 52\,000 \\
4B generation 3 & $+5.20$ & $+0.55$ to $+1.06$ & $+0.60$ & $+0.00$ to $+1.25$ & $-2.3$ to $+2.8$ & $2.8$ & 720 to 2\,700 \\


==> generated/transfer-ratios.tex <==
Iterative protocol, 4B (one run) & $+25.87$ & $+2.75$ & 0.11 & inconclusive \\
Iterative protocol, 8B (one run) & $+33.93$ & $+6.25$ & 0.18\textsuperscript{a} & excluded \\
Training material, outcome first (three seeds) & $+17.16$ & $+3.50$ & 0.20 & supported \\
Training material, all verified (three seeds) & $+51.33$ & $+1.83$ & 0.04 & supported \\
Training material, productive actions (three seeds) & $+53.55$ & $+1.83$ & 0.03 & supported \\
Training material, one per task (three seeds) & $+46.88$ & $+0.83$ & 0.02 & supported \\


==> generated/unit-audit.tex <==
\nolinkurl{vim-transfer/decision/decision-eval-exam.json} & 8 & task & not stated & recorded \\
\nolinkurl{vim-transfer/decision/decision-eval-unseen.json} & 7 & task & not stated & recorded \\
\nolinkurl{vim-transfer/decision/secondary-eval-exam.json} & 4 & task & not stated & recorded \\
\nolinkurl{vim-transfer/decision/secondary-eval-unseen.json} & 3 & task & not stated & recorded \\
\nolinkurl{vim-transfer/decision/student-only-decision-eval-exam.json} & 1 & task & not stated & recorded \\
\nolinkurl{vim-transfer/loop/loop.json} & 13 & task & not stated & recorded \\
\nolinkurl{vim-transfer/loop/rerun-4b.json} & 9 & attempt slot & exact one-sided paired sign test over tasks & bounds only \\
\nolinkurl{vim-transfer/loop/rerun-8b.json} & 9 & attempt slot & exact one-sided paired sign test over tasks & bounds only \\
\nolinkurl{vim-transfer/loop/seed-replicates.json} & 59 & attempt slot & one-sided exact sign test over tasks, pooled over seeds & bounds only \\
\nolinkurl{vim-transfer/loop/seed-replicates.json} & 14 & attempt slot, summed over training seeds & one-sided exact sign test over tasks, pooled over seeds & no (shared tasks and champion) \\
\nolinkurl{vim-transfer/retention/retention.json} & 18 & task & not stated & recorded \\


==> generated/vim-transfer-attempts.tex <==
section by section & Qwen3-4B & 8204 & 10.0\% & 1026 & 231 \\
section by section & Qwen3.8-27B-FP8 & 4095 & 81.1\% & 1026 & 944 \\
outcome first & Qwen3-4B & 3688 & 3.1\% & 467 & 36 \\
outcome first & Qwen3.8-27B-FP8 & 1868 & 72.2\% & 467 & 410 \\


==> generated/vim-transfer-secondary.tex <==
outcome first vs all verified & 21/5 & 0.0025 & $+1.67$ [$+0.25$, $+3.08$] \\
productive actions vs all verified & 7/5 & 0.774 & $+0.00$ [$-0.83$, $+0.83$] \\
one per task vs all verified & 2/8 & 0.109 & $-1.00$ [$-1.92$, $-0.17$] \\


==> generated/vim-transfer-t1.tex <==
all verified & 94 & 705/1128 (62.5\%) & 126/1128 & 82/1, \ensuremath{8.7\times 10^{-24}} & $+51.33$ [$+44.68$, $+58.16$] \\
one per task & 94 & 642/1128 (56.9\%) & 113/1126 & 79/3, \ensuremath{1.9\times 10^{-20}} & $+46.98$ [$+39.72$, $+54.17$] \\
productive actions & 94 & 723/1128 (64.1\%) & 119/1128 & 84/1, \ensuremath{2.2\times 10^{-24}} & $+53.55$ [$+46.28$, $+60.46$] \\
shuffled requests & 94 & 9/1128 (0.8\%) & 133/1128 & 2/26, \ensuremath{3.0\times 10^{-6}} (two-sided) & $-10.99$ [$-16.31$, $-6.38$] \\
outcome first & 51 & 127/612 (20.8\%) & 22/612 & 25/0, \ensuremath{3.0\times 10^{-8}} & $+17.16$ [$+11.11$, $+23.69$] \\


==> generated/vim-transfer-table.tex <==
all verified & 3359 (2699) & 22 (6, 6, 10) & 10 & 0/1174 & 10/0, 0.00098 & 10/0, 0.00098 \\
one per task & 771 (629) & 10 (5, 2, 3) & 6 & 0/1188 & 6/0, 0.016 & 6/0, 0.016 \\
productive actions & 3359 (2699) & 22 (10, 4, 8) & 11 & 0/1187 & 11/0, 0.00049 & 11/0, 0.00049 \\
shuffled requests & 3359 (2699) & 0 (0, 0, 0) & 0 & 0/1177 & -- & -- \\
outcome first & 1100 (1014) & 42 (14, 11, 17) & 25 & 0/1175 & 24/0, \ensuremath{6.0\times 10^{-8}} & 25/0, \ensuremath{3.0\times 10^{-8}} \\

